On the Privacy of dK-Random Graphs

Real social network datasets provide significant benefits for understanding phenomena such as information diffusion or network evolution. Yet the privacy risks raised from sharing real graph datasets, even when stripped of user identity information, are significant. Previous research shows that many graph anonymization techniques fail against existing graph de-anonymization attacks. However, the specific reason for the success of such de-anonymization attacks is yet to be understood. This paper systematically studies the structural properties of real graphs that make them more vulnerable to machine learning-based techniques for de-anonymization. More precisely, we study the boundaries of anonymity based on the structural properties of real graph datasets in terms of how their dK-based anonymized versions resist (or fail) to various types of attacks. Our experimental results lead to three contributions. First, we identify the strength of an attacker based on the graph characteristics of the subset of nodes from which it starts the de-anonymization attack. Second, we quantify the relative effectiveness of dK-series for graph anonymization. And third, we identify the properties of the original graph that make it more vulnerable to de-anonymization.

==> sections/dataset.tex <==
\section{Experimental Setup}

\ainote{Not sure what of this text will stay, but need to build the connection with the previous sections.}
Our objective is to quantify the graph-anonymization benefits of graph generation techniques that preserve the dk distribution. 
To this end, we select a number of real network datasets (presented in Section~\ref{sec:datasets}) and extract their various dk-distributions. 
We then generate random graphs from these dk distributions (as presented in Section~\ref{sec:dk_random_graphs}) to play the roles of auxiliary and anonymized graphs.
Note that a pair of auxiliary and anonymized graph (that is, generated in a particular dk-space and for a specific degree distribution) are connected by a set of shared nodes, as presented above. 
We then apply the methodology described in the previous section to measure how well machine learning techniques can match node identities from the auxiliary and the anonymized graphs. 
%Note that both the auxiliary and the anonymized graphs are generated based on dk-graph generation techniques. 


\subsection{Network Datasets}
\label{sec:datasets}

%The dk graph generators are given the respective degree distributions and other graph characteristics (such as clustering coefficient) of a set of real networks. 
We chose five publicly available datasets that represent real social networks of various types. 
\texttt{fb107}~\cite{leskovec2012learning} represents social circles of an ego in Facebook. 
%%\ainote{huh? it's only the contacts of one person + their contacts? Why is this a relevant network?}.
%%\shnote{This would give us good points on comparison when we talk about degree one nodes in the experiments, because ego network lack such nodes}
\texttt{caGrQc}~\cite{leskovec2007graph} is a co-authorship network between the authors of papers submitted to the scientific domain of general relativity and quantum cosmology.
%\ainote{in what context and domain? Who are the nodes, what are the edges?}.
\texttt{soc-anybeat}~\cite{Fire2012} is an interaction network available in the Anybeat online community, which is a public gathering place across the world.
\texttt{soc-gplus}~\cite{networkrepo} is a follower network from Google+.
Finally, \texttt{web-frwikinews-user-edits}~\cite{networkrepo} is a discussion network of Wikipedia pages. 
Table~\ref{tbl:dataset} summarizes the graph statistics of these datasets.


\begin{table*}[bthp]
	
	\caption{%Basic graph properties, Note that all the graphs are undirected, Clustering $(\bar{C})$ depicts the average of local clustering coefficient of nodes, and transitivity $(C)$ is the fraction of all possible triangles in the graph.
Graph properties of the real network datasets. All graphs are undirected. density $(\bar{d})$ is the fraction of all possible edges, transitivity $(C)$ is the fraction of triangles of all possible triangle in the network while the clustering $(\bar{C})$ is the average local clustering coefficients of the nodes. degree-assortativity $(r)$ measures the similarity of relations depending on the associated node degree. avg-path-length $(\kappa)$ depicts the average shortest path length between any pairs of nodes
%\ainote{what? Is the average path length? Why change the terminology, then?} 
and degree-1 represents the percentage of nodes in the network with degree exactly 1. 
%\ainote{One way to reduce the width of the table is to move the terminology in the caption and leave only the notation as column headers.} %\ainote{Do we use the notations? Do we need them?}
}
	\label{tbl:dataset}
	\begin{tabular}{|r|r|r|r|r|r|r|r|r|}
		\hline 
		Network & $|N|$ & $|E|$ & $\bar{d}$ & $C$ & $\bar{C}$ & $r$ &  $\kappa$ & degree-1 (\%)\\ 
		\hline \hline
		fb107 & 1034 &  26749 & 0.1000 &  0.2534 & 0.5264  & 0.4316 &  2.9517 & 1.45 \\ 
		\hline 
		caGrQc & 5242 & 14496 & 0.0011 & 0.3621 & 0.5295 & 0.6592 & 3.8047 & 22.83 \\ 
		\hline 
		soc-anybeat & 12645 & 49132 & 0.0006 & 0.0073 & 0.2037 & -0.1234 & 3.1715 & 49.51 \\ 
		\hline 
		soc-gplus & 23628 &  39194 & 0.0001 & 0.0012 & 0.1741 & -0.3885 & 4.0277 & 69.16 \\ 
		\hline 
		web-frwikinews & 25042 & 68679 & 0.0002 & 0.0001 & 0.1133 & -0.2544 & 2.9666 & 33.52 \\ 
		\hline 
	\end{tabular} 
\end{table*}




\subsection{dk-Random Graphs}
\label{sec:dk_random_graphs}
\ainote{To re-write:} dk-graphs define a set of graphs that represent the respective dk-distribution.
dk-random graphs are a subset of dk-graphs that define the maximum-entropy ensemble~\cite{orsini2015quantifying}.
Each dk-random graph has the same probability ($\frac{1}{N_d}$) to be drawn from the population of dk-graphs.
$N_d$ is the size of dk-space, which can be calculated approximately for $d \leq 2$ \cite{bianconi2007entropy,barvinok2013number}.  
%However, a rigorous mathematical proof about $N_d$ is lacking at the moment~\cite{orsini2015quantifying}. 
\ainote{This, though, is irrelevant for us, as we really have d=2 as maximum, even for 2.5k.} However, $N_d$ increases significantly as d increases, and incur large memory requirements for the computation~\cite{sala2010measurement}.
\ainote{I find this paragraph extraordinarily opaque. Have a look at Sala's paper for a crystal clear presentation of the dk graphs. Can we write something of the same level of clarity (at least?)}
\shnote{Check, I refer sala about the size and computation on dk-spaces}
\ainote{My point was not about referring Sala. My point was about writing style -- in their paper (and typically in Ben Zhao's papers) complicated things are presented in a way that are easy to understand and read. This is a really important skill to build.}
\shnote{got it. bdw dk-random graphs are presented in the introduction}

For our experiments, we generate $m=4$ dk-random graphs for each subgraph $G_1$ and $G_2$ per dk-space. 
We use three graph generation techniques proposed in previous work. 

1k-graphs are graphs randomly chosen from the space of graphs with a given degree distribution. 
To generate them, we used Orbis~\cite{mahadevan2006systematic} with dk randomizing rewiring.  
The algorithm works by rewiring random pairs of edges from the original graph in order to preserve the 1k-distribution.
%As suggested in~\cite{mahadevan2006systematic}, we allow a sufficient number of initial isomorphic rewirings, and then follow a subsequent set of rewirings to verify that the 1k-series remain intact.
This method results in an unbiased sampling of 1k-graphs with a significant variation of properties, such as degree-correlations and clustering~\cite{orsini2015quantifying}. 
%	Also, it's required to perform a sufficient number of 1k-preserving rewiring to find the global optima of 1k-convergence. 

%	\item[--] 
The 2k-graphs preserve a given joint degree distribution, including the degree-correlations. 
We used dK-targeting \ainote{do you mean the ' in the following?:} \shnote{The method stated in the literature is dK-targeting $d'K$-preserving}
$d'K$-preserving rewiring based on Metropolis dynamics as implemented by Gjoka et al.~\cite{gjoka201325k}. 
2k-graphs are generated by beginning with any 1k-graph and rewiring edges only if such modifications move the graph closer to 2k-series.

%\item[--] 
For generating 2.5k graphs we used an improved version of the Metropolis method (MCMC) proposed in~\cite{gjoka201325k}. 
2.5k graphs are 2K graphs that preserve a given clustering coefficient in addition to the dk-2 distribution. 
This method starts by adding triangles to a 2k graph to reach a clustering coefficient threshold and then destroys them to recreate the desired joint degree distribution. 
For generating these graphs, we chose the parameters to ensure uniform sampling over the dk-space. (It has been shown experimentally~\cite{orsini2015quantifying} that the number of dk-swaps required for the MCMC method is $O(|E|)$).
%	the dk-swap Markov chain is after its mixing time is reached

%\end{itemize}

\ainote{To rewrite this paragraph. I moved it from where it was. Is it still relevant? If so, should we make a claim about the datasets having power law distributions?} We believe that they are close to uniform samples since they exhibit power-law degree distributions.
It is shown that the dk-randomizing swapping approach using Metropolis method guarantees to have uniform sampling in power-law graphs~\cite{orsini2015quantifying}. 
The number of node pairs that we could generate over the dk-space increases quadratically, $\mathcal{O}(mn^2)$, where $n$ is the size of dk-random graph.




\begin{table*}[bthp]
	\centering
	\caption{Basic statistics of generated node pairs over dk-spaces under the overlap choices of Random, High Degree and BFS-trees (rooted in the highest degree node BFS-HD and, respectively, a random node, BFS-R). We generated a total of $\approx$ 1 billion identical and non-identical node pairs over three dk-spaces of the five real social network datasets, and took  $364K$ balanced samples.}
	% 1044.8 billions, 364800 samples
	\label{tbl:sample_space}
	\begin{tabular}{|c|c|r|r|r|r|c|}
		\hline
		\multicolumn{2}{|c|}{\multirow{2}{*}{Network}} & \multicolumn{4}{c|}{No. of generated node pairs (\textit{millions})} & \multirow{2}{*}{No. of balanced samples $\ell$}\\
		\cline{3-6}
		\multicolumn{2}{|c|}{} & Random&High-Degree&BFS--HD&BFS--R & \\
		\hline
		\multirow{3}{*}{fb107} & 1k & 0.85 & 0.84 & 0.88 & 0.88 & 12800 
		%270, 265, 277, 275 
		\\
		\cline{2-7}
		& 2k & 0.85 & 0.84 & 0.88 & 0.89 & 12800 
		% 266, 264, 276, 276
		\\
		\cline{2-7}
		& 2.5k & 0.86 & 0.85 & 0.88 & 0.89 & 12800
		% 271, 270, 277, 278
		\\
		\hline
		\hline
		\multirow{3}{*}{caGrQc} & 1k & 2.36 & 2.30 & 3.92 & 3.98 & 12800 
		% 620, 560, 973, 1015
		\\
		\cline{2-7}
		& 2k & 3.10 & 3.07 & 4.96 & 3.75 & 12800 
		% 830, 806, 1240, 1252
		\\
		\cline{2-7}
		& 2.5k & 3.13 & 3.07 & 4.96 & 5.00 & 12800 
		% 815, 781, 1240, 1252
		\\
		\hline
		\hline
		\multirow{3}{*}{soc-anybeat} & 1k & 10.95 & 10.85 & 24.35 & 26.06 & 32000\\
		\cline{2-7}
		& 2k & 10.65 & 12.60 & 24.50 & 26.20 & 32000\\
		\cline{2-7}
		& 2.5k & 11.18 & 13.56 & 24.55 & 26.20 & 32000 \\
		\hline
		\hline
		\multirow{3}{*}{soc-gplus} & 1k & 10.55 & 11.53 & 45.04 & 43.47 & 32000\\
		\cline{2-7}
		& 2k & 12.33 & 11.40 & 45.06 & 49.80 & 32000 \\
		\cline{2-7}
		& 2.5k & 12.56 & 10.40 & 45.06 & 49.80 & 32000 \\
		\hline
		\hline
		\multirow{3}{*}{web-frwikinews} & 1k & 23.58 & 23.16 & 46.80 & 46.67 & 32000\\
		\cline{2-7}
		& 2k & 22.63 & 25.16 & 46.87 & 46.72 & 32000 \\
		\cline{2-7}
		& 2.5k & 21.55 & 25.43 & 46.87 & 46.72 & 32000 \\
		\hline
		% etc. ...
	\end{tabular}
\end{table*}



\begin{figure}[bthp]
	\centering
	\includegraphics[width=\linewidth]{images/d-measure/d_distance_G_bar}
	\caption{
	%\ainote{Remove the title from the picture itself (see top). Check all the other plots and do the same.} 
	Average structural distance between the original network and a dk-generated network 
	%\ainote{does this matter: [overlap choice = BFS-Tree(Highest-Degree)]}
	using D-measure~\cite{schieber2017quantification}. The structural distance D-measure is calculated between the original network and 4 different instances of its corresponding dk-random graphs and the average value is reported, along with the confidence intervals}
	\label{fig:d_distance_all}
\end{figure}


\subsection{Characteristics of dK-generated Graphs}

We confirmed that the 4 instances of dk-generated graphs for every set of parameters are distinct. 
We also measured the structural distance between the original graph and the generated graphs. 
For this, we used D-measure~\cite{schieber2017quantification}, a dissimilarity metric that quantifies the topological differences based on network node dispersion (NND). 
%which stands out against metrics using Hamming and graph-edit distance. 
A low D-measure ($\approx 0$) suggests that graphs have the same distance distribution, the same NND and the same $\alpha$-centrality vector~\cite{schieber2017quantification}. 
%Non-isomorphic graphs have a D-measure of 1.
Non-zero D-measure indicates graphs are non-isomorphic, and the maximum that it could reach is 1.

Figure~\ref{fig:d_distance_all} shows the average distance between each of the real networks \ainote{why do we have only 3 networks in here and not all 5?}
\shnote{The R process is being killed in other two datasets, probably out of memory}
and its corresponding dk-generated graph in each of the dK spaces we consider. 
The plot suggests two observations: First, for sparser graphs, the generated networks are relatively close to the original dataset (e.g., for the \texttt{soc-anybeat} dataset the average D-measure is $\approx 0.325$, while for \texttt{fb107}, the average D-measure $\approx 0.415$). This observation is supported by intuition, as sparse graphs tend to have lower node degrees, thus relatively few opportunities for rewiring to lead to significantly different topology. Second, 
\ainote{I don't see the same variation in the new barplot compared to the line plot yesterday -- check the correctness of the pics, perhaps? I remember more difference between dk spaces for some networks, while now is very close to 0}
\shnote{It's the same, the variation is small $\approx +/-\ 0.1$} the transition from 1k to 2k and 2.5k present a relatively good difference over dense graphs (see confidence intervals in the network fb107, average D-measure $\approx 0.415$).
However, the dk-space graphs are closer to the original topology (lower D-measure) when the graphs are sparse (), and the transition from dk-spaces is not significant.


\ainote{I am not sure we will need this subsection in the end. I wonder if some of these results should be included in the next section, when we discuss the results. It seems that the observations are the following (please correct/expand):
1) the four instances of generated graphs are different from each others and different from the original dataset; 
2) the distance between the original graph and the generated graphs is smaller for sparse networks than for dense -- which makes sense, intuitively. This intuitively may mean that they are also easier to de-anonymize. To make sure we discuss this point in the next section. 
3) the overlaps have different proportions of degree-1 nodes, and since those carry less information, we could then connect this fact with prediction success (I hope?). 
}

\ainote{Note that the discussion about overlaps is more related to the ML experimental framework than to th edk-graphs. So then I wonder what is the best place for Table 2 and also the figure on degree-1 nodes in overlap.}
\shnote{They fit in the next section as an intro}

%\ainote{Why are we looking at this plot? What was our initial motivation for doing this measurement? Weren't we trying to verify that we are generating different graphs than the original? Did we succeed? Weren't we also trying to make sure that we generate 4 different instances of the dk-generated graphs? Can we confirm that somehow? (maybe in text). Also, this plot does not seem to be extremely relevant for the results -- it is perhaps one that could be cut and kept for a journal version or a more detailed technical report.}


%\shnote{First, I calculate properties of dk-graphs to see the variation of them (I still have them in appendix, commented). I take D-measure to see how closer/furthest dk-graphs from the original, and to see the difference of dk-convergence between sparse and dense networks.}

%\ainote{this is a very complicated way of commenting a plot:}



We also observe \ainote{Where? Not in Figure~\ref{fig:d_distance_all}, I don't think} \shnote{This is from the graph metrics calculated for dk-graphs, in the appendix, huge table to show?}
that the subgraphs with the overlap of BFS-Tree (Highest Degree) of soc-anybeat, soc-gplus and web-frwikinews-user-edits graphs are significantly constrained by the degree distribution upon the graph generation process. 
Thus, even 1k-random graphs approximate them reasonably well.
%(see the graph properties at Appendix \ref{sec:appendix}).
%(Table \ref{tbl:dk_soc-anybeat}, \ref{tbl:dk_soc-gplus} and \ref{tbl:dk_web-frwikinews-user-edits}). 
However, the subgraphs of fb107 and caGrQc are least constrained; 1k-random graphs approximate them poorly, and dk-series convergence is at 2k space.
%(Table \ref{tbl:dk_fb107} and \ref{tbl:dk_caGrQc}).

%\ainote{I am unsure of the value of Figure~\ref{fig:d_distance_all} because of a few points: what is the maximum value for D-measure? without this information, it is impossible to compare the graphs. The difference between the graphs seems to be relatively small -- 0.10, whatever that means.}
%\shnote{D-measure is from 0 to 1, but such small difference says a lot, what I want to convince is; sparse dk-graphs are closer to the original than dense graphs. It's indirectly about the dk-space.}


%\begin{itemize}
%\item[--] About dk-convergence (Figure \ref{fig:d_distance_all}): 
%
%%\literature{
%%".. Results for the Petster (C) network show that models considering 2.1k are closer to the real network than 2k models; this can be the case of an outlier network ..." } \cite{schieber2017quantification}
%\end{itemize}

Figures~\ref{fig:low_degree_bfs1} and~\ref{fig:low_degree_deg} highlight the properties of degree-1 nodes over the overlap subgraphs across original and dk-spaces. 
%We observe that they are dominated by a large percentage of low-degree (i.e degree-1) nodes when the graphs become sparse.
%We identify that when the graph becomes more sparse, they display negative degree-assortativity (Figure \ref{tbl:dataset}), by having negative correlations with similar magnitude node degree pairs. 
%As a consequence, there is a large percentage of low-degree (i.e degree-1) nodes and, they give rise to preferential attachment model exhibit in large social graphs.
We note that subgraphs with the overlap of both choices have shown a significant variation of the proportion of degree-1 nodes over the dk-spaces when the graphs become sparse (Figure~\ref{fig:low_degree}).
Beside that, overlap subgraph of high degree nodes have the majority of degree-1 nodes when comparing with the other choice.
As an example, soc-gplus shows $86.25\%$ of degree-1 nodes in the former choice (Figure~\ref{fig:low_degree_deg}), while it decreases to $43.33\%$ in the latter (Figure~\ref{fig:low_degree_bfs1}).
This is due to the less connectivity among high degree nodes in the original graph.
% that show positive assortativity.
The more interesting observation, though, is that the proportion of degree-1 nodes in the 1k-space degrades significantly comparing with other dk-spaces over the overlap subgraph of BFS-Tree (see the networks of soc-anybeat, soc-gplus and web-frwikinews in Figure~\ref{fig:low_degree_bfs1})

%When considering the network soc-anybeat, node-induced subgraph of the overlap in 1k-space shows only $20.08 \%$ proportion of low degree nodes, while it increases more than $3x$ times in 2k and 2.5k spaces.
%We have seen the neighbors of the highest degree node are less likely form clusters when comparing with the neighbors of a lower degree node in higher dk-spaces.
%But the opposite can be seen in 1k-space when the original graph is sparse.
%Because 1k-graphs are least constrained only by the degree distribution, it's not a strict requirement to link low-degree nodes to hubs.
%Therefore, we note that 1k generators would tend to produce many isolated degree-1 nodes connected to one another.


%\begin{table*}[htb!]
%	\caption{Average of proportion (\%) degree-1 users over original and dk-space graphs, overlap $\alpha=0.2$}
%	\label{tbl:dk_low_deg}
%\begin{tabular}{|c|c|c|c|c|c|}
%	\hline 	
%	Overlap choice & Network & Original (\%) & 1k (\%) & 2k (\%)  & 2.5k (\%)\\ 
%	\hline \hline 
%	\multirow{5}{*}{BFS-Tree (Highest Degree)}& fb107 & 2.285 & 2.125 & 2.285 & 2.285  \\ 
%	& caGrQc & 29.175 & 20.5 & 29.2 & 29.2 \\
%	& soc-anybeat & 53.33 & 53.01 & 53.33 & 53.33 \\
%	& soc-gplus & 63.525 & 63.51 & 63.525 & 63.525 \\
%	& web-frwikinews & 37.665 & 37.59 & 37.665 & 37.665 \\ \hline
%	\multirow{5}{*}{High Degree} & fb107 & 2.69 & 1.895 & 2.69 & 2.69 \\
%	& caGrQc & 34.865 & 24.145 & 34.925 & 34.925 \\
%	& soc-anybeat & 53.87 & 53.495 & 53.87 & 53.87 \\
%	& soc-gplus & 74.585 & 74.51 & 74.585 & 74.585 \\
%	& web-frwikinews & 43.93 & 43.79 & 43.93 & 43.93 \\ \hline
%\end{tabular} 
%\end{table*}

%\begin{table*}[t]
%	\caption{Average percentage (\%) of nodes with degree one in the overlap subgraph, overlaps are taken over $8$ sample instances with the overlap choice of BFS-Tree (Highest Degree)}
%	\begin{minipage}[b]{0.475\linewidth}
%%		\centering
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline 	
%			Network & Original GS (\%) & 1k (\%) & 2k (\%)  & 2.5k (\%)\\ 
%			\hline \hline 
%			fb107 & 0 & 0 & 0 & 0  \\ 
%			caGrQc & 10.21 & 12.84 & 10.75 & 8.9 \\
%			soc-anybeat & 57.22 & 20.08 & 99.925 & 99.925 \\
%			soc-gplus & 43.33 & 40.98 & 99.85 & 99.84 \\
%			web-frwikinews & 33.3 & 19.78 & 99.91 & 99.925 \\ \hline
%		\end{tabular}
%		\label{tbl:low_degree_bfs1}
%	\end{minipage}
%	\begin{minipage}[b]{0.425\linewidth}
%%		\centering
%		\includegraphics[scale=0.35]{images/low_degree_bfs1}
%		\label{fig:low_degree_bfs1}
%	\end{minipage}
%\end{table*}
%
%\begin{table*}[t]
%	\caption{Average percentage (\%) of nodes with degree one in the overlap subgraph, overlaps are taken over $8$ sample instances with the overlap choice of High Degree}
%	\begin{minipage}[b]{0.475\linewidth}
%		%		\centering
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline 	
%			Network & Original GS (\%) & 1k (\%) & 2k (\%)  & 2.5k (\%)\\ 
%			\hline \hline 
%			fb107 & 9.38 & 12.4 & 12.5 & 11.3 \\
%			caGrQc & 57.35 & 57.42 & 62.1 & 67.05 \\
%			soc-anybeat & 68.11 & 60.62 & 64.13 & 64.45 \\
%			soc-gplus & 86.25 & 89.48 & 88.8 & 89.47 \\
%			web-frwikinews & 66.85 & 85.67 & 85.68 & 81.81 \\ \hline
%		\end{tabular}
%		\label{tbl:low_degree_deg}
%	\end{minipage}
%	\begin{minipage}[b]{0.425\linewidth}
%		%		\centering
%		\includegraphics[scale=0.35]{images/low_degree_deg}
%		\label{fig:low_degree_deg}
%	\end{minipage}
%\end{table*}

\begin{figure}[bthp]
	\centering
	\subfloat[High Degree]{
		\includegraphics[scale=0.2]{images/low_degree_deg}
			\label{fig:low_degree_deg}
	}
	\hspace{0mm}
	\subfloat[BFS-HD]{
		\includegraphics[scale=0.2]{images/low_degree_bfs1}
			\label{fig:low_degree_bfs1}
	}
	\caption{Average percentage of nodes with degree 1 in the overlap subgraph across dk-spaces (including GS). The overlaps are averaged over 8 sample instances in each dk space for two overlap strategies: highest-degree nodes (a) and BFS rooted in the highest degree node (b). Figure also shows the confidence intervals of average measurements.}
	\label{fig:low_degree}
\end{figure}





==> sections/methodology.tex <==
\section{Methodology}
\label{sec:methodology}
In this section, we present the methodology to benchmark the privacy in $dK$-Random graphs.
The notion of privacy is assumed as a way of protecting node-level anonymity in the original graph.
We employ a similar data model, assumptions, and notations of an existing work~\cite{Sharad2016benchmark} that provides a machine learning framework (as presented in Section \ref{sec:experimental-framework})  for the analysis of anonymization schemes.
Further, we use $dK$-based graph generation techniques (presented in Section \ref{sec:dk_random_graphs}) as our anonymization method and 
mount a machine learning based de-anonymization attack on $dK$-graphs to facilitate our benchmark.
The purpose is to find the bijection between two unlabeled graphs whose edge sets are correlated~\cite{pedarsani2011privacy}.
To support the learning algorithm, we create feature vectors using the node signatures presented in Section \ref{sec:node-signatures}.


%We explain the common threat model employed in our benchmark (as presented in Sections \ref{sec:threat-model} and \ref{sec:experimental-framework}), which is followed by the measurements to quantify anonymity (as presented in Section \ref{sec:random-forest-classification}) in $dK$ random graphs.
%Also, we briefly discuss $dK$ graph construction methods in Section \ref{sec:dk_random_graphs}. 


%\ainote{Ideally, here we would give a very high level intuition of what we're going to do, and in the following subsections we go into details. This high level intuition is simply meant to put the pieces together.}
%\shnote{Updated.}

\subsection{Threat Model}
\label{sec:threat-model}
%More often, the problem of re-identification of nodes in an anonymized graph is mapped to the identification of corresponding nodes in an 
%auxiliary graph.
%This is further being reduced to the variations of \textit{graph isomorphism problem} \cite{corneil1970efficient}.
We follow the general threat model used in~\cite{Sharad2016benchmark} to measure the success of a de-anonymization attack.
This model proceeds on matching the node sets (unlabeled) of two graphs at an attacker's disposal.
As an example, an attacker has two unlabeled networks of individuals in an organization that represent the communication patterns (e.g., email) and friendship information available from an online social network. 
Both networks have been anonymized by removing the original labels of nodes and perturbing edges.
However, these graphs can be structurally overlapping, in that some individuals are present in both graphs, even if their identities have been removed.  
The task is to find a bijective mapping between the two subsets of nodes in the two graphs that correspond to the individuals present in both networks. 
The efficacy of this mapping is being measured by the rate of correctly identifying the overlap set of nodes that are common to the two graphs, as in~\cite{Sharad2016benchmark}, and also measuring the nodes correctly identified as not the same. 
It's straightforward to see when more nodes are common to the two graphs (i.e. the size of overlap $\alpha$ increases), it's easier to identify more nodes in the overlap.
More importantly, we keep a low $\alpha$ value constant over our experiments.

%\ainote{correct?}

\subsection{Experimental Framework}
\label{sec:experimental-framework}
%Our goal is to approximate the adversarial knowledge, where the strength of given attack could be tuned by the parameters (i.e. size $\alpha$ and choice) of the overlap.
We assume that any adversary has an anonymized graph $G_{san}$ that could be associated with an auxiliary graph $G_{aux}$ for the re-identification attack. 
As discussed before, $G_{san}$ could be the anonymized version of the communication (e.g., email) graph, while $G_{aux}$ is a part of the friendship network. %, where this selection could be interchanged.
%\ainote{we need to go back to the intuition presented with the two graphs above. Which one, email or friendship, is $G_{aux}$, for example? Does it really matter which is which?}
%\shnote{Updated.}

In order to model this scenario, we split a real dataset graph $G=(V,E)$ into two subgraphs $G_1=(V_1,E_1)$ and $G_2=(V_2,E_2)$, such that $V_1 \subset V$, $V_2 \subset V$ and $V_1 \cap V_2 = $V_\alpha$, where $V_\alpha \ne \phi$. 
%\ainote{unit problem here? size of a set is integer, this formula makes it a fraction. I wonder if you mean $\alpha$, in fact, and not $V_{alpha}$:} 
The size of the overlap is measured by the Jaccard coefficient of two subsets: $\alpha=\frac{|V_1 \cap V_2|}{|V_1 \cup V_2|}$ . 

In order to experiment with various strengths of the attack in addition to the value of $\alpha$, we build $V_\alpha$ in four different ways: i)~as a random collection of nodes from the original graph $G$ (Random)
%(\ainote{this is the place for introducing the notations}); 
ii)~by selecting the highest degree nodes from $G$ (High Degree); iii)~ by building a breadth-first-search tree starting from a randomly selected node in $G$ (BFS-R); and iv)~by building a breadth-first-search tree starting from the highest degree node in $G$ (BFS-HD). 
While other alternatives are certainly possible, these four approaches cover an important set of realistic assumptions on the attacker.  

\ainote{I am thinking that $\alpha$ and overlap structure are in fact part of the threat model. Maybe not with the formalism, which should be presented here, but the intuition should be there -- perhaps, the more nodes common to the two graphs are, the easier to identify more nodes. }
\shnote{check the ending of sec 3.1, Updated.}


\begin{figure}[t]
	\centering
	\includegraphics[scale=0.1]{images/dk_mining_flow}
	\caption{Graph mining system flow to generate node pairs with the ground truth of identical and non-identical pairs. %\ainote{I don't understand this:}The instances of $G_{aux}$ and $G_{san}$ pairs approximate the auxiliary and anonymized graphs at attacker's disposal.\shnote{This is being explained in the text, just a recall, but we can remove it from the caption}
	}
	\label{fig:dkminingflow}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.5]{images/ndd-demo}
	\caption{Example node signature that defines a feature vector of bin size b = 2, and the number of bins 2. Each bin value corresponds to the number of nodes that have degree in the bin range, such that $i^{th}$ bin holds the nodes in the degree ($d_i$) range $i \times b \leq d_i < (i+1) \times b$. If the degree exceeds the maximum range, such nodes are included in the last bin. Furthermore, both 1-hop binned NDD and 2-hop binned NDD are merged. As an example, node $j$ has no 1-hop neighbor nodes that have degree in the range of $1-2$, and one 2-hop neighbor node with node degree in the range of $1-2$. The node value in the example represents the node's degree.}
	\label{fig:ndd_demo}
\end{figure}


\subsection{$dK$-Random Graphs}
\label{sec:dk_random_graphs}
\shnote{Important para. Check. Need more clarity, Help !!! if can please read the first para of sec 3.3.2 - True Friends paper}
In an optimistic scenario, an attacker has access to a part of the original graph (e.g., $G_1$) as auxiliary data and to an unperturbed subgraph (e.g., $G_2$) as anonymized data.
However, this is unrealistic, since researchers and practitioners are well aware now that without perturbing the structure of the graph, even with identifiable node and edge attributes removed, there is no anonymity~\cite{Sharad2016benchmark}.
Hence, in order to reproduce a realistic scenario, we anonymize both $G_1$ and $G_2$ graphs.
We assume an instance of this anonymized graphs could be the furthest for being attacked~\cite{Sharad2016benchmark}.

Then, we split them with the same overlap parameters (i.e. size $\alpha$ and choice of the overlap) to play the roles of auxiliary $(G_{aux})$ and anonymized $(G_{san})$ graph versions (see Figure \ref{fig:dkminingflow}).
In fact, we approximate $G_{aux}$ by having a different instance of an anonymized subgraph.

This allows us to sample node pairs from the overlapping sets for which we know the ground truth.


%For graph anonymization, we chose to generate $dK$-graphs from the respective node degree distributions of the real graphs.

%\ainote{one paragraph here that described briefly the dK graph generators and their motivation.}
%\shnote{I'm working on this motivation...Finished.}
Recall that, our problem is to measure the effectiveness of anonymization schemes.
We approach this problem by synthetically generating random graphs based on degree-correlations modeled by $dK$-series.
In fact, it's shown that we could regenerate realistic networks by analyzing the degree-correlation~\cite{mahadevan2006systematic}.
This setting allows us to measure the level of privacy of the original graph under different utility constraints.
%Indirectly, we could also measure the level of privacy of the original graph under different utility constraints.


%\ainote{I do not know what and why is relevant from here:}
%\shnote{check Fig 1, this is the explanation for the final parts}
%Each $dK$-space is represented by a set of $m$ number of generated $dK$-graphs, which are local to $G_1$ and $G_2$.
%We assume that an instance of this set could be the furthest for being attacked.
%Therefore, we split the anonymized graphs with the same overlap parameters to produce the versions of $G_{aux}$ auxiliary and $G_{san}$ graphs.
%Such that we believe that an adversary uses $G_{aux}$ as prior knowledge to attack $G_{san}$ in which this selection can be interchanged~\cite{Sharad2016benchmark}.


We use $dK$-series as a set of descriptive statistic measurements to capture the original graph structure at multiple levels of detail~\cite{sala2011sharing}.
In fact, $dK$-series summarizes the structure of a graph from the degree distribution of a subgraph pattern of size $d$. 
Full analysis of a particular graph begins by generating $dK$-random graphs with fixed average node degree ($0K$-graphs), then with fixed 
degree distribution ($1K$-graphs), then with fixed joint degree distribution ($2K$-graphs), then with fixed interconnectivity of triplets of nodes 
($3K$-graphs), and so on up to the $NK$-graph, reproducing the original graph.  
Intermediate steps in the series can be defined, such as, the $2.5K$ graph, which is a relaxed version of $3K$-graphs that reproduces both joint degree distribution and degree-dependent clustering 
coefficient \cite{gjoka201325k}.  

%\ainote{to here. }



%\shnote{This is an important text; explain the way we approximate auxiliary and anonymized graphs in the framework, I am not sure whether this para fits here, might be best at the end of sec 3.2, without the notion of dK, but just describing as "anonymization"}
%For our experiments, we generate $m=4$ number of $dK$-random graphs for each subgraph $G_1$ and $G_2$ per $dK$-space.
%Then, we split them to produce subgraphs with the same overlap parameters (i.e. size $\alpha$ and choice of the overlap) as the initial partition of the graph $G$. 
%This set of subgraphs play the roles of auxiliary $(G_{aux})$ and anonymized $(G_{san})$ versions (see Figure \ref{fig:dkminingflow}).
%We assume that an instance of this set could be the furthest for being attacked. 
%\ainote{we have a terminology problem here because we end up anonymizing the anonymized graph. Can we do better?}
%\ignore{
%Note that a pair of auxiliary $(G_{aux})$ and anonymized $(G_{san})$ graph (that is, generated in a particular dk-space and for a specific degree distribution) are connected by a set of shared nodes, as presented above.} 
 
We use three graph generation techniques (for 1K, 2K, and 2.5K, respectively) proposed in previous work. 
For our experiments, we generate $m=4$ number of $dK$-random graphs for each subgraph $G_1$ and $G_2$ per $dK$-space.

$1K$-graphs are graphs randomly chosen from the space of graphs with a given degree distribution. 
To generate them, we used Orbis~\cite{mahadevan2006systematic} with $dK$ randomizing rewiring.  
The algorithm works by rewiring random pairs of edges from the original graph in order to preserve the $1K$-distribution.
As suggested in~\cite{mahadevan2006systematic}, we allow a sufficient number of initial isomorphic rewirings, and then follow a subsequent set of rewirings to verify that the 1k-series remain intact.
This method results in an unbiased sampling of $1K$-graphs with a significant variation of properties, such as degree-correlations and clustering~\cite{orsini2015quantifying}. 
%	Also, it's required to perform a sufficient number of 1k-preserving rewiring to find the global optima of 1k-convergence. 

%	\item[--] 
The $2K$-graphs preserve a given joint degree distribution, including the degree correlations. 
We used $dK$-targeting $d'K$-preserving rewiring based on Metropolis dynamics as implemented by Gjoka et al.~\cite{gjoka201325k}. 
$2K$-graphs are generated by beginning with any $1K$-graph and rewiring edges only if such modifications move the graph closer to $2K$-series.

%\item[--] 
For generating $2.5K$ graphs we used an improved version of the Metropolis method (MCMC) proposed in~\cite{gjoka201325k}. 
$2.5K$ graphs are $2K$ graphs that preserve a given clustering coefficient in addition to the $2K$ distribution. 
This method starts by adding triangles to a $2K$ graph to reach a clustering coefficient threshold and then destroys them to recreate the desired joint degree distribution. 
For generating these graphs, we chose the parameters to ensure uniform sampling over the $dK$-space. (It has been shown experimentally~\cite{orsini2015quantifying} that the number of dk-swaps required for the MCMC method is $O(|E|)$).
%	the dk-swap Markov chain is after its mixing time is reached

%\end{itemize}
We limit our study for the $dK$-spaces of $1K,\ 2K$ and $2.5K$ on the classification of various graph metrics because algorithms exist that almost surely sample uniformly at random elements of the corresponding set of graphs.  
No such algorithms exist for steps higher in the series.


\subsection{Node Signatures}
\label{sec:node-signatures}
%In large social-graphs, the degree distribution captures a set of important features of the topology \cite{orsini2015quantifying}.
%Many anonymized schemes try to preserve the degree distribution as much as possible, to avoid the effect of serious utility degradation \cite{sharad2016learning}.
%In fact, it's observed that a large proportion of nodes in a graph are uniquely distinguishable from the neighborhood degree distribution (NDD) \cite{hay2007anonymizing}.
Since we are employing machine-learning techniques to "label" nodes in a graph, we need to represent the nodes as vectors of features. 
We use neighborhood degree distribution (NDD) as part of the signature of a node, as done in~\cite{sharad2016learning}.   
NDD uses the degree distribution of neighbors to describe a node~\cite{Sharad2016benchmark}.
This decision is supported by the observation that a large proportion of nodes in a graph are uniquely distinguishable by their NDD~\cite{Sharad2016benchmark}.
%Indeed, NDD captures the degree distribution of related ego-nets.


We build the signature of a node as a vector with the following structure. 
We apply a binning strategy to aggregate each node's 1-hop and 2-hop NDD (Figure~\ref{fig:ndd_demo}).
In our experiments, we set the number of bins to $21$ and the size of bins to $50$ for the calculation of binned NDD. 
We employ the same binning technique used in Sharad \cite{Sharad2016benchmark} because it was shown empirically to capture the high degree variations of large social graphs.
In fact, binning increases matching accuracy, but any error would be tolerated over the comparison of classification results.
Importantly, we use the same binning strategy over all experiments.
This statistical quantification captures the aggregate structure of ego networks which is expected to be robust against edge perturbation due to anonymization~\cite{sharad2016learning}.





\subsection{Random Forest Classification}
\label{sec:random-forest-classification}
%We have $2 \times m$ instances of such $G_{aux}$ and $G_{san}$ pairs, that are used to sample node pairs with the ground truth.
%The ground truth explains whether any pair of nodes are identical or not.
%To benchmark our results, we also generate pairs of node signatures from the subgraphs $G_1$ and $G_2$, denoted as the population $GS$.
%Figure \ref{fig:dkminingflow} presents the steps of generating identical and non-identical node pairs, while Table \ref{tbl:sample_space} summarizes the statistics of the population of samples.


We generate examples for the training phase of the de-anonymization attack to measure how well machine learning techniques can match node identities from the anonymized $(G_{san})$ and the auxiliary $(G_{aux})$ graphs.
These examples support the given learning algorithm to uncover artifacts in the anonymization method~\cite{sharad2016learning}.


We have $2 \times m$ instances of $G_{aux}$ and $G_{san}$ pairs that are used to sample node pairs with the ground truth.
The ground truth explains whether any pair of nodes are identical or not.
In most cases, we have an unbalanced dataset, with the degree of imbalance depending on the overlap parameter $\alpha$, where the majority is non-identical node pairs.
We use reservoir sampling technique~\cite{haas2016data}
%\ainote{need real reference here. Do not cite wikipedia, please.} %\footnote{https://en.wikipedia.org/wiki/Reservoir\_sampling} 
to take $\ell$ balance sub-samples from the population $S$, and SMOTE algorithm as an over-sampling technique for each sub-sample.
%Each sample is split into training and testing sets. 
Each sample is trained by a forest of 100 random decision tress that allows to learn features and the accuracy is being measured on unseen examples in the same sample space.
Gini-index is used as an impurity measure for the random forest classification.
Given the size $\alpha$ and choice of the overlap, we measure the quality of the classifier on the task of differentiating two nodes as identical or not. 
We use $2 \times m \times \ell \times 100$ number of decision trees per $dK$-space for the learning process in each graph space.
%In addition, multiple weak learners as a combination, would result a performance improvement over the classification task \cite{sharad2014automated}.
Table \ref{tbl:sample_space} summarizes the statistics of the sample population.



%\subsection{De-anonymity Measure}
We then measure the accuracy of a classifier to determine the indistinguishability of identical and non-identical pair from a random pair of nodes.
Accuracy is being measured by the distribution of F1-score $\in \mathbb{R}_{0,1}$, which is the harmonic mean between the precision and recall of a local classifier.
The success rate of de-anonymization depends upon the quality of many weak classifiers that provide rough predictions.

\begin{table*}[bthp]
	
	\caption{%Basic graph properties, Note that all the graphs are undirected, Clustering $(\bar{C})$ depicts the average of local clustering coefficient of nodes, and transitivity $(C)$ is the fraction of all possible triangles in the graph.
Graph properties of the real network datasets. All graphs are undirected. density $(\bar{d})$ is the fraction of all possible edges, transitivity $(C)$ is the fraction of triangles of all possible triangle in the network while the clustering $(\bar{C})$ is the average local clustering coefficients of the nodes. degree-assortativity $(r)$ measures the similarity of relations depending on the associated node degree. avg-path-length $(\kappa)$ depicts the average shortest path length between any pairs of nodes
%\ainote{what? Is the average path length? Why change the terminology, then?} 
and degree-1 represents the percentage of nodes in the network with degree exactly 1. 
%\ainote{One way to reduce the width of the table is to move the terminology in the caption and leave only the notation as column headers.} %\ainote{Do we use the notations? Do we need them?}
}
	\label{tbl:dataset}
	\begin{tabular}{|r|r|r|r|r|r|r|r|r|}
		\hline 
		Network & $|N|$ & $|E|$ & $\bar{d}$ & $C$ & $\bar{C}$ & $r$ &  $\kappa$ & degree-1 (\%)\\ 
		\hline \hline
		fb107 & 1034 &  26749 & 0.1000 &  0.2534 & 0.5264  & 0.4316 &  2.9517 & 1.45 \\ 
		\hline 
		caGrQc & 5242 & 14496 & 0.0011 & 0.3621 & 0.5295 & 0.6592 & 3.8047 & 22.83 \\ 
		\hline 
		soc-anybeat & 12645 & 49132 & 0.0006 & 0.0073 & 0.2037 & -0.1234 & 3.1715 & 49.51 \\ 
		\hline 
		soc-gplus & 23628 &  39194 & 0.0001 & 0.0012 & 0.1741 & -0.3885 & 4.0277 & 69.16 \\ 
		\hline 
		wikinews & 25042 & 68679 & 0.0002 & 0.0001 & 0.1133 & -0.2544 & 2.9666 & 33.52 \\ 
		\hline 
	\end{tabular} 
\end{table*}


\begin{table*}[bthp]
	\centering
	\caption{Basic statistics of generated node pairs over dk-spaces under the overlap choices of Random, High Degree and BFS-trees (rooted in the highest degree node BFS-HD and, respectively, a random node, BFS-R). We generated a total of $\approx$ 1 billion identical and non-identical node pairs over three dk-spaces of the five real social network datasets, and took  $364K$ balanced samples.}
	% 1044.8 billions, 364800 samples
	\label{tbl:sample_space}
	\begin{tabular}{|c|c|r|r|r|r|c|}
		\hline
		\multicolumn{2}{|c|}{\multirow{2}{*}{Network}} & \multicolumn{4}{c|}{No. of generated node pairs (\textit{millions})} & \multirow{2}{*}{No. of balanced samples $\ell$}\\
		\cline{3-6}
		\multicolumn{2}{|c|}{} & Random&High-Degree&BFS--HD&BFS--R & \\
		\hline
		\multirow{3}{*}{fb107} & 1k & 0.85 & 0.84 & 0.88 & 0.88 & 12800 
		%270, 265, 277, 275 
		\\
		\cline{2-7}
		& 2k & 0.85 & 0.84 & 0.88 & 0.89 & 12800 
		% 266, 264, 276, 276
		\\
		\cline{2-7}
		& 2.5k & 0.86 & 0.85 & 0.88 & 0.89 & 12800
		% 271, 270, 277, 278
		\\
		\hline
		\hline
		\multirow{3}{*}{caGrQc} & 1k & 2.36 & 2.30 & 3.92 & 3.98 & 12800 
		% 620, 560, 973, 1015
		\\
		\cline{2-7}
		& 2k & 3.10 & 3.07 & 4.96 & 3.75 & 12800 
		% 830, 806, 1240, 1252
		\\
		\cline{2-7}
		& 2.5k & 3.13 & 3.07 & 4.96 & 5.00 & 12800 
		% 815, 781, 1240, 1252
		\\
		\hline
		\hline
		\multirow{3}{*}{soc-anybeat} & 1k & 10.95 & 10.85 & 24.35 & 26.06 & 32000\\
		\cline{2-7}
		& 2k & 10.65 & 12.60 & 24.50 & 26.20 & 32000\\
		\cline{2-7}
		& 2.5k & 11.18 & 13.56 & 24.55 & 26.20 & 32000 \\
		\hline
		\hline
		\multirow{3}{*}{soc-gplus} & 1k & 10.55 & 11.53 & 45.04 & 43.47 & 32000\\
		\cline{2-7}
		& 2k & 12.33 & 11.40 & 45.06 & 49.80 & 32000 \\
		\cline{2-7}
		& 2.5k & 12.56 & 10.40 & 45.06 & 49.80 & 32000 \\
		\hline
		\hline
		\multirow{3}{*}{wikinews} & 1k & 23.58 & 23.16 & 46.80 & 46.67 & 32000\\
		\cline{2-7}
		& 2k & 22.63 & 25.16 & 46.87 & 46.72 & 32000 \\
		\cline{2-7}
		& 2.5k & 21.55 & 25.43 & 46.87 & 46.72 & 32000 \\
		\hline
		% etc. ...
	\end{tabular}
\end{table*}






